Mutual Information of a class of Poisson-type Channels using Markov Renewal Theory

The mutual information (MI) of Poisson-type channels has been linked to a filtering problem since the 70s, but its evaluation for specific continuous-time, discrete-state systems remains a demanding task. As an advantage, Markov renewal processes (MrP) retain their renewal property under state space filtering. This offers a way to solve the filtering problem analytically for small systems. We consider a class of communication systems $X \to Y$ that can be derived from an MrP by a custom filtering procedure. For the subclasses, where (i) $Y$ is a renewal process or (ii) $(X,Y)$ belongs to a class of MrPs, we provide an evolution equation for finite transmission duration $T>0$ and limit theorems for $T \to \infty$ that facilitate simulation-free evaluation of the MI $\mathbb{I}(X_{[0,T]}; Y_{[0,T]})$ and its associated mutual information rate (MIR). In other cases, simulation cost is reduced to the marginal system $(X,Y)$ or $Y$. We show that systems with an additional $X$-modulating level $C$, which statically chooses between different processes $X_{[0,T]}(c)$, can naturally be included in our framework, thereby giving an expression for $\mathbb{I}(C; Y_{[0,T]})$. Our primary contribution is to apply the results of classical (Markov renewal) filtering theory in a novel manner to the problem of exactly computing the MI/MIR. The theoretical framework is showcased in an application to bacterial gene expression, where filtering is analytically tractable.

==> Bibliography/manual-bibliography.tex <==
\begin{thebibliography}{9}

\bibitem{Laport:LaTeX}
L.~Lamport,
  \emph{\LaTeX: A Document Preparation System,} 
  Addison-Wesley, Reading, Massachusetts, USA, 2nd~ed., 1994. 

\bibitem{GMS:LaTeXComp}
F.~Mittelbach, M,~Goossens, J.~Braams, D.~Carlisle, and
C.~Rowley, \emph{The {\LaTeX} Companion,} Addison-Wesley,
Reading, Massachusetts, USA, 2nd~ed., 2004.

\bibitem{oetiker_latex}
T.~Oetiker, H.~Partl, I.~Hyna, and E.~Schlegl, \emph{The Not So Short
  Introduction to {\LaTeX2e}}, version 5.06, Jun.~20, 2016. [Online].
  Available: \url{https://tobi.oetiker.ch/lshort/}

\bibitem{typesetmoser}
S.~M. Moser, \emph{How to Typeset Equations in {\LaTeX}}, version 4.6,
  Sep. 29, 2017. [Online]. Available:
  \url{http://moser-isi.ethz.ch/manuals.html#eqlatex}

\bibitem{IEEE:pdfsettings}
IEEE, \emph{Preparing Conference Content for the IEEE Xplore Digital
  Library.} [Online]. Available:
  \url{http://www.ieee.org/conferences_events/conferences/organizers/pubs/preparing_content.html}

\bibitem{IEEE:AuthorToolbox}
IEEE, \emph{Author Digital Toolbox.} [Online.] Available:
  \url{http://www.ieee.org/publications_standards/publications/authors/authors_journals.html}

\end{thebibliography}

==> Proofs/Prop-UniformBoundDRI.tex <==
 The sMk-elements associated with biochemical reactions often have densities with support on $\Rzero$. For this case, the following proposition provides easily verifiable sufficient conditions for the application of Theorem \ref{thm:MrP-Limits}.
 \begin{proposition}
     Let $|\stsp|<\infty$. The sMk-densities $\elsmkd{y}{z}$ ($y,z \in E$) be continuous a.e. with finite number of discontinuities, d.R.i. functions with support $\Rzero$. The embedded Markov chain be irreducible recurrent. If $\lim_{t \to \infty} \frac{\elsmkd{y}{z}}{\elembMat{y}{z}-\elSMK{y}{z}}< \infty$ for all $y,z \in \stsp$ with $\elembMat{y}{z}>0$, then $\sup_{y \in \stsp} \sup_{v \geq 0} \Lambda(t,y)< \infty$.
     \label{proposition:UniformBoundDRI}
 \end{proposition}

\begin{IEEEproof}[Proof of proposition \ref{proposition:UniformBoundDRI}]
    Since all d.R.i. functions are bounded and continuous a.e. \cite{asmussen2008applied} (p. 154, Prop. 4.1 (i)). Hence $v \mapsto \Lambda_{z}(y,v)$ is bounded on finite intervals and continuous a.e. For all $y,z \in \stsp$ and $v \geq 0$ it holds $\Lambda_{z}(y,v) \leq \sum_{z \in \stsp} \Lambda_{z}(y,v) = \frac{\elSoujd{y} (v)}{\elSurvD{z}(v)}$, the hazard function associated with $\elSoujD{z}$. This hazard function is also continuous a.e. and boundet on finite intervals (as a finite sum of functions with these properties). So $\Lambda_{z}(y,v)$ is bounded if $\lim_{t \to \infty} \frac{\elSoujd{y} (v)}{\elSurvD{z}(v)}<\infty$. Due to finite number of discontinuity points the limit may exist on $[0,\infty]$. We rewrite $v \mapsto \elSoujD{z}(v) = \sum_{y \in \stsp} \elSMK{z}{y}(v) = \sum_{y \in \stsp}  \elembMat{z}{y}\frac{\elSMK{z}{y}(v)}{\elembMat{z}{y}}$, which is a proper mixture of the probability distributions $\{\frac{\elSMK{z}{y}(v)}{\elembMat{z}{y}} \mid y \in \stsp \}$. Since $\lim_{t \to \infty} \frac{\elsmkd{y}{z}}{\elembMat{y}{z}-\elSMK{y}{z}}< \infty$ for all $y,z \in \stsp$ with $\elembMat{y}{z}>0$ we obtain $ \lim_{t \to \infty} \frac{\elSoujd{y} (v)}{\elSurvD{z}(v)}< \infty$ by \cite{block2003initial} (Theorem 2.1).
\end{IEEEproof}
Note that \cite{block2003initial} (Theorem 2.1) can be used with less restrictive assumptions.
